HepData reloaded: reinventing the HEP data archive

We describe the status of the HepData database system, following a major re-development in time for the advent of LHC data. The new HepData system benefits from use of modern database and programming language technologies, as well as a variety of high-quality tools for interfacing the data sources and their presentation, primarily via the Web. The new back-end provides much more flexible and semantic data representations than before, on which new external applications can be built to respond to the data demands of the LHC experimental era. The HepData re-development was largely motivated by a desire to have a single source of reference data for Monte Carlo validation and tuning tools, whose status and connection to HepData we also briefly review.

==> acat-hepdata-preamble.tex <==
\usepackage{graphicx}
\usepackage{xspace}
\usepackage{amsmath,amssymb,bm}
\usepackage{cite}
\usepackage{rotating}
\usepackage{relsize}
\usepackage{snapshot}
\usepackage{booktabs}
\usepackage[labelfont=bf]{caption}
%\usepackage{underscore}
\usepackage[italic]{hepparticles}
\usepackage{hepnames,hepunits}
\usepackage{subfigure}
\usepackage{sidecap} % Allow cpations to appear next to a figure

%%% To work with JHEP.cls, (x)color.sty needs this work-around:
\usepackage{xcolor}
\makeatletter
\let\default@color\current@color
\makeatother

%%% I'm not sure if we really want to format URLs \smaller ...
\usepackage{url}
\makeatletter
\def\url@smallerstyle{%
  \@ifundefined{selectfont}{\def\UrlFont{\smaller}}{\def\UrlFont{\smaller}}}
\makeatother
\urlstyle{smaller}


\IfFileExists{microtype.sty}{%
  \RequirePackage{microtype}%
  %\RequirePackage[tracking=true]{microtype}%
  %\UseMicrotypeSet[tracking]{smallcaps}%
  %\SetTracking{encoding=*,shape=sc}{30}
}{}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\DeclareMathOperator{\det}{det}

\newcommand{\EqRef}[1]{equation~\eqref{#1}\xspace}
\newcommand{\SecRef}[1]{section~\ref{#1}\xspace}
\newcommand{\TabRef}[1]{Table~\ref{#1}\xspace}
\newcommand{\FigRef}[1]{Figure~\ref{#1}\xspace}
\newcommand{\TabsRef}[1]{Tables~\ref{#1}\xspace}
\newcommand{\FigsRef}[1]{Figures~\ref{#1}\xspace}

\newcommand{\p}{\ensuremath{\vec{p}}\xspace}
\newcommand{\pzero}{\ensuremath{\vec{p}_0}\xspace}
\newcommand{\pprime}{\ensuremath{\vec{p}^{\,\prime}}\xspace}
\newcommand{\N}[1]{\ensuremath{N^{\mspace{0.5mu}(\mspace{-0.5mu}#1)}}\xspace}
\newcommand{\Nn}[2]{\ensuremath{N_{\,#1}^{\mspace{0.5mu}(\mspace{-0.5mu}#2)}}\xspace}
\newcommand{\Nmin}[1]{\ensuremath{N_\text{min}^{\mspace{0.5mu}(\mspace{-0.5mu}#1)}}\xspace}
\newcommand{\Nmax}[1]{\ensuremath{N_\text{max}^{\mspace{0.5mu}(\mspace{-0.5mu}#1)}}\xspace}
\newcommand{\Ndf}{\ensuremath{N_\text{df}}\xspace}
\newcommand{\Ptilde}{\ensuremath{\mathbf{\tilde{P}}}\xspace}
\newcommand{\ptilde}{\ensuremath{\tilde{p}}\xspace}
\newcommand{\vptilde}{\ensuremath{\vec{\tilde{p}}}\xspace}
\newcommand{\Ipseudo}{\ensuremath{\tilde{\mathcal{I}}}\xspace}
\newcommand{\DeltaOf}[1]{\ensuremath{\Delta\mspace{0.75mu}#1}\xspace}
\newcommand{\vcoeff}{\ensuremath{\vec{c}}\xspace}
\newcommand{\vcoeffb}{\ensuremath{\vec{c}^{(b)}}\xspace}
\newcommand{\coeffb}[1]{\ensuremath{c^{(b)}_{#1}}\xspace}
\newcommand{\vval}{\ensuremath{\vec{v}}\xspace}
\newcommand{\vvalb}{\ensuremath{\vec{v}^{(b)}}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\chisqNdf}{\ensuremath{\chi^2\!/\Ndf}\xspace}
\newcommand{\nCr}[2]{\ensuremath{\parenths{\colvec{#1 \\ #2}}}\xspace}
\newcommand{\wO}{\ensuremath{w_{\mathcal{O}}}\xspace}
\newcommand{\alphaS}{\ensuremath{\alpha_\text{s}}\xspace}
\newcommand{\sqrts}{\ensuremath{\sqrt{s}}\xspace}
\newcommand{\pT}{\ensuremath{p_\perp}\xspace}
\newcommand{\pTlead}{\ensuremath{{p_{\perp}^\text{\:lead}}}\xspace}
\newcommand{\pTleadmin}{\ensuremath{{p_{\perp}^\text{\:lead, min}}}\xspace}
\newcommand{\pTleadmax}{\ensuremath{{p_{\perp}^\text{\:lead, max}}}\xspace}
\newcommand{\LambdaQCD}{\ensuremath{\Lambda_\text{QCD}}\xspace}
\newcommand{\ofOrder}[1]{\ensuremath{\mathcal{O}(#1)}\xspace}
\newcommand{\order}[1]{\ensuremath{\mathcal{O}(#1)}\xspace}
\newcommand{\kbd}[1]{{\smaller{\texttt{#1}}}}
\newcommand{\stat}{\ensuremath{\text{stat}}\xspace}
\newcommand{\sys}{\ensuremath{\text{syt}}\xspace}

\newcommand{\xparagraph}[1]{\par\vspace{2mm}\noindent\emph{#1}\quad}
\newcommand\centerAlign[1]{%
   \raisebox{-0.5\height}{#1}%
}

\def\PARJ#1{\ensuremath{\text{PARJ(#1)}}}
\def\PARP#1{\ensuremath{\text{PARP(#1)}}}
\def\MSTJ#1{\ensuremath{\text{MSTJ(#1)}}}

%%% A very visible way of displaying TODOs:
\definecolor{todoboxcolor}{rgb}{1.0,0.6,0.6}
\newcommand{\TODO}[1]{\par\medskip \noindent%
\colorbox{todoboxcolor}{TODO: \parbox[t]{6.5cm}{#1}}%
\medskip\par}

\definecolor{todoneboxcolor}{rgb}{1.0,0.9,0.9}
\newcommand{\TODONE}[1]{\par\medskip \noindent%
\colorbox{todoneboxcolor}{TODONE?: \parbox[t]{6.5cm}{#1}}%
\medskip\par}


%%% Some names, to use a consistent spelling throughout the document:
\def\aleph{ALEPH\xspace}
\def\delphi{DELPHI\xspace}
\def\tasso{TASSO\xspace}
\def\opal{OPAL\xspace}
\def\lthree{L3\xspace}
\def\cdf{CDF\xspace}
\def\dzero{D\O\xspace}
\def\ATLAS{ATLAS\xspace}
\def\cms{CMS\xspace}

\def\lep{LEP\xspace}
\def\lepi{LEP~1\xspace}
\def\lhc{LHC\xspace}
\def\tevatron{Tevatron\xspace}
\def\rhic{RHIC\xspace}
\def\hera{HERA\xspace}
\def\sld{SLD\xspace}

\def\fnal{FNAL\xspace}
\def\cern{CERN\xspace}

\def\mcnet{MCnet\xspace}
\def\pdg{PDG\xspace}

\def\runi{Run-\textsmaller{I}\xspace}
\def\runii{Run-\textsmaller{II}\xspace}
\def\runiia{Run-\textsmaller{II}a\xspace}
\def\runiib{Run-\textsmaller{II}b\xspace}

\def\Cpp{C\raisebox{0.2ex}{\smaller++}\xspace}

\def\fortran{Fortran\xspace}
\def\pythia{Pythia\xspace}
\def\phojet{Phojet\xspace}
\def\pythiasix{Pythia~6\xspace}
\def\pythiaeight{Pythia~8\xspace}
\def\herwig{Herwig\xspace}
\def\herwigsix{Herwig~6\xspace}
\def\herwigpp{Herwig\raisebox{0.1ex}{\smaller++}\xspace}
\def\sherpa{Sherpa\xspace}
\def\alpgen{AlpGen\xspace}
\def\charybdis{Charybdis\xspace}
\def\jimmy{Jimmy\xspace}
\def\rivet{Rivet\xspace}
\def\rivetgun{Rivetgun\xspace}
\def\professor{Professor\xspace}
\def\fastjet{FastJet\xspace}
\def\hepmc{HepMC\xspace}
\def\agile{AGILe\xspace}
\def\hztool{HZTool\xspace}
\def\numpy{NumPy\xspace}
\def\scipy{SciPy\xspace}
\def\minuit{Minuit\xspace}
\def\pyminuit{PyMinuit\xspace}
\def\python{Python\xspace}

\def\jade{Jade\xspace}
\def\durham{Durham\xspace}

\def\gof{GoF\xspace}

